Least squares estimation in nonstationary nonlinear cohort panels with learning from experience

We discuss techniques of estimation and inference for nonstationary nonlinear cohort panels with learning from experience, showing, inter alia, the consistency and asymptotic normality of the nonlinear least squares estimator used in empirical practice. Potential pitfalls for hypothesis testing are identified and solutions proposed. Monte Carlo simulations verify the properties of the estimator and corresponding test statistics in finite samples, while an application to a panel of survey expectations demonstrates the usefulness of the theory developed.

==> general_recursion.tex <==
 {\Huge Responses}

\subsection{The general recursion}
Suppose the agent, in order to form expectations about next periods inflation, uses an additional (scalar) regressor $x_t$, i.e. agents' prediction of $y_t$ is given by $\pi_{t,s}(\gamma) \coloneqq a_{t-1,s}(\gamma)x_t$, where
\begin{equation}
\begin{split}
  r_{t,s}(\gamma)                  & = r_{t-1,s}(\gamma) + \gamma_{t,s}(\gamma) (x_t^2 - r_{t-1,s}(\gamma)) \\
  a_{t,s}(\gamma)               & = a_{t-1,s}(\gamma) + \gamma_{t,s}(\gamma) \frac{x_t}{r_{t,s}(\gamma)} (y_t - a_{t-1,s}(\gamma)x_t). 
  \end{split}
\end{equation}
Note that $x_t$ and $a_{t-1,s}(\gamma)$ depend on each other in a non-trivial way. 

\begin{remark}
    For $\gamma = 1$, we obtain $a_{t,t-s}(\gamma) = \sum_{j=0}^{s-\floor{\gamma}}x_{t-j}y_{t-j}/ \sum_{j=0}^{s-\floor{\gamma}}x_{t-j}^2$, i.e. the OLS estimator. More generally, $a_{t,t-s}(\gamma)$ is a weighted least-squares estimator of the population regression coefficient $\Ex[xy]/\Ex[x^2]$, assuming stationarity and that the expectations exist. 
\end{remark}

Because $a_{t,s}(\gamma)$ determines the non-linear regression function, the statistical properties of it (e.g. moments up to order four) are crucial for the analysis. In particular, our analysis in the MS makes it clear that a theory of the NLS estimator requires, among other things, for
\[
\frac1{\nu_n}\sum_{t=u+1}^n\sum_{s=l}^u \tilde\pi^2_{t,t-s}(\gamma)
\quad \text{ and } \quad
\frac1{\sqrt\nu_n}\sum_{t=u+1}^n\sum_{s=l}^u \tilde\pi_{t,t-s}(\gamma)\eps_{t,t-s},
\]
 a ULLN and a FCLT, respectively, where, as in the MS, a {\it tilde} indicates cohort-demeaning; i.e.  $\tilde \pi_{t,s}(\gamma) = \pi_{t,s}(\gamma) - \bar\pi_t(\gamma),$ $\bar\pi_{t}(\gamma) \coloneqq \frac{1}{m}\sum_{s=l}^u \pi_{t,t-s}(\gamma) = x_t\bar a_{t-1}(\gamma);$ hence $\tilde \pi_{t,s}(\gamma) = x_t(a_{t-1,s}(\gamma) - \bar a_{t-1}(\gamma)) = x_t \tilde a_{t-1,s}(\gamma)$. 

To give you a first flavour of the difficulties we encountered when attempting at doing so, it is instructive to consider the explicit solution of the recursion given by
\[
a_{t,t-s}(\gamma) = \sum_{j=\floor{\gamma}}^s\rd\hat\kappa_{j,s,t}(\gamma)\bk \frac{x_{t-s+j}y_{t-s+j}}{r_{t-s+j,t-s}(\gamma)},\qquad \rd\hat\kappa_{j,s,t}(\gamma)\bk \coloneqq \frac{\gamma}{j}\prod_{i=j+1}^sf_{i,s,t}(\gamma),
\]
where 
$$f_{i,s,t}(\gamma) = 1-\frac{\gamma}{i}\frac{x_{t-s+i}^2}{r_{t-s+i,t-s}(\gamma)},$$
and the (stochastic) weights $\hat\kappa_{j,s,t}(\gamma)$ satisfy the conventions $\hat\kappa_{s,s,t}(\gamma) \coloneqq \frac{\gamma}{s}$ and  $\hat\kappa_{\floor{\gamma},s,t}(\gamma) \coloneqq  \prod_{i=\floor{\gamma}+1}^sf_{i,s,t}(\gamma)$. The recursion of the regressor second-moment can be solved similarly
\[
r_{t,t-s}(\gamma)= \sum_{j=\floor{\gamma}}^s\bl\kappa_{j,s}(\gamma)\bk x_{t-s+j}^2, \quad \bl\kappa_{j,s}(\gamma)\bk \coloneqq \frac{\gamma}{j}\prod_{i=j+1}^s\left(1-\frac{\gamma}{i}\right),
\]
with the (deterministic) weights satisfying $\kappa_{s,s}(\gamma) \coloneqq \frac{\gamma}{s}$, $\kappa_{\floor{\gamma},s}(\gamma) \coloneqq  \prod_{i=\floor{\gamma}+1}^s(1-\frac{\gamma}{i})$, defined in the MS. Therefore, contrary to the case in the MS, the weights of $a_{t,s}(\gamma)$ are ($1$) stochastic and ($2$) depend in addition on the second recursion $r_{t,s}(\gamma)$, which highly complicates the analysis. 

\begin{remark}
    For $x_t = 1$, we obtain $a_{t,t-s}(\gamma) = \sum_{j=\floor{\gamma}}^s\kappa_{j,s}(\gamma)y_{t-s+j}$, i.e. the recursion analysed in the MS. 
\end{remark}

A proof strategy would build on first showing that the recursion $r_{t,s}(\gamma)$, which is seen to be an estimator of the regressor second moment, is uniformly close to $\Ex[x^2]$. This can then be used to argue that the stochastic $\hat\kappa_{j,s,t}(\gamma)$ behave (in a certain probabilitic sense) similar to the deterministic weights $\kappa_{j,s}(\gamma)$ uniformly in $\gamma \in \Gamma$; the latter are well understood by the use of our results from the MS. The intuition stems from
\[
\kappa_{j,s}(\gamma) = \frac{\gamma}{j}\prod_{i=j+1}^s\Ex\left[ f_{i,t,s}(\gamma) \mid r_{t-s+i,t-s}(\gamma) = \Ex[x^2]\right].
\]
More formally, the idea of "replacing" the recursion $r_{t,s}(\gamma)$ in the conditional expectation of the preceding display with $\Ex[x^2]$ is based on the following conjecture that, as agents grow older (i.e. $t-s \rightarrow \infty$), the recursion $r_{t,s}(\gamma)$ tends to $\Ex[x^2]$ uniformly in $\gamma$.

\begin{conjecture}
If $x_t$ is stationary and strongly mixing, then  $$\ssup\limits_{\gamma\in \Gamma}|r_{t,t-s}(\gamma)-\Ex[x^2]| \rightarrow_{a.s.} 0$$ as $s \rightarrow \infty$ such that $t-s \rightarrow \infty$ for $\Gamma \subset (1/2,\infty)$.
\end{conjecture}

{\footnotesize {\bf  Sketch of a Proof.} Note that $r_{t,t-s}(\gamma)-\Ex[x^2] = \sum_{j=\floor{\gamma}}^s\kappa_{j,s}(\gamma)(x_{t-s+j}^2-\Ex[x^2]).$ A point-wise SLLN is based on the idea that if $\mmax_{j}\kappa_{j,s}(\gamma) = O(b_s)$, $b_s \downarrow 0$, with $b_s\sum_{j}^s(x_{t-s+j}^2-\Ex[x^2]) = o_{a.s}(1)$, then also the weighted sum is $o_{a.s}(1)$. Now,
\[
\mmax\limits_{\floor{\gamma} \leq j \leq s}\kappa_{j,s}(\gamma) =  \begin{cases}
			\displaystyle\frac{\gamma}{s}, &  \gamma \geq 1\\
            \kappa_{1,s}(\gamma), & \gamma \in (1/2,1),
		 \end{cases}
\]
where
\(
\kappa_{1,s}(\gamma) = \gamma\prod_{j=2}^s(1-\gamma/i) = \frac{\Gamma(s-\gamma+1)}{\Gamma(s+1)\Gamma(2-\gamma)} = \frac{\gamma}{s^\gamma}(1+o(1)).
\)
If $\gamma \geq 1$, then $\frac1{s}\sum_{j=1}^s(x_{t-s+j}^2-\Ex[x^2]) \rightarrow_{a.s.} 0$ by a standard SLLN for stationary ergodic time series. If $\gamma \in (1/2,1)$, then,  by the Marcinkiewicz-Zygmund type SLLN of Rio (1995, Thm 1, {\it Ann. Probab.}), $\frac1{s^\gamma}\sum_{j=1}^s(x_{t-s+j}^2-\Ex[x^2]) \rightarrow_{a.s.} 0,$ $\gamma \in (1/2,1)$. To see that the SLLN holds uniformly we can exploit the stochastic Lipschitz-continuity of $r_{t,s}(\gamma)$ (see Lemma A0 ($iii$) in the MS) and \citet[Lemma 1]{andrews:92}.
}

This conjecture leads us to believe that $\sum_{j=\floor{\gamma}}^s \hat\kappa_{j,s,t}(\gamma) = 1+o_p(1)$ (the equality is exact for $x_t = 1$), such that
\[
\tilde a_{t,t-s}(\gamma) = a_{t,t-s}(\gamma) - \underbrace{\bar a_t}_{\simeq \Ex[xy]/\Ex[x^2]} \simeq \sum_{j=\floor{\gamma}}^s\kappa_{j,s}(\gamma)\frac{x_{t-s+j}y_{t-s+j}-\Ex[xy]}{\Ex[x^2]},
\]
where the term on the right-hand side can be analysed using the theory developed in the MS. However, similar to \cite{mayer:22}, to make the above approximations rigorous we have to control the behaviour of higher-order moments of partial sums involving as summands products of random variables (i.e. the $\hat\kappa_{j,s,t}(\gamma)$) and, contrary to \cite{mayer:22}, these arguments have to hold uniformly over $\gamma \in \Gamma$. This additional layer of complexity is therefore left to future research.


\newpage

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> proofs/test.tex <==
Without loss of generality, assume $\gamma <  \gamma_2$. 
 \begin{align}
  {\sf D}_m(\gamma_1) = \sum_{t=u+1}^n\sum_{s=l}^u\Ex[(a_{t,t-s}(\gamma_1)-a_{t,t-s}( \gamma_2))^2] 
\end{align}
where the expectations are independent of $t$ and given by
\begin{align*}
    \Ex[(a_{t,t-s}(\gamma_1)-a_{t,t-s}( \gamma_2))^2] = \,& \sum_{i,j=\floor{\gamma_1}}^s\kappa_{j,s}(\gamma_1)\kappa_{i,s}(\gamma_1)c(i-j)\\
&+\sum_{i,j=\floor{ \gamma_2}}^s\kappa_{j,s}( \gamma_2)\kappa_{i,s}( \gamma_2)c(i-j)\\
&-2\sum_{i=\floor{ \gamma_2}}^s\sum_{j=\floor{\gamma_1}}^s\kappa_{i,s}( \gamma_2)\kappa_{j,s}(\gamma_1)c(i-j) \\
= \,& (\kappa_s(\gamma_1)-\tilde\kappa_s( \gamma_2))^\Tr M(\kappa_s(\gamma_1)-\tilde\kappa_s( \gamma_2)
\end{align*}
 where $\kappa_s(\gamma_1) \coloneqq (\kappa_{\floor{\gamma_1},s}(\gamma_1),\kappa_{\floor{\gamma_1}+1,s}(\gamma_1).\dots,\kappa_{s,s}(\gamma_1))^\Tr$ and $$\tilde\kappa_s( \gamma_2) = (0_{\floor{\gamma_1}-\floor{ \gamma_2}}^\Tr,\kappa_s( \gamma_2)^\Tr)^\Tr$$
 are $(s-\floor{\gamma_1}+1)\times 1$ vectors while 
  $$
 M_s = [c(i-j)]_{0 \leq i,j \leq s-\floor{\gamma_1}}.
 $$
 is a $(s-\floor{\gamma_1}+1)\times (s-\floor{\gamma_1}+1)$ positive definite Toeplitz matrix with minimum eigenvalue $\infty > \mmin\limits_{1\leq s\leq u}\lambda_1(M_s)\geq\lambda>0$. Hence,
\begin{align}\nonumber
    {\sf D}_m(\gamma_1) \geq \lambda(1-u/n)\sum_{s=l}^u |\kappa_s(\gamma_1)-\tilde\kappa_s( \gamma_2)|^2,
\end{align}
with
\[
|\kappa_s(\gamma_1)-\tilde\kappa_s( \gamma_2)|^2 =
 \sum_{j=\floor{\gamma_1}}^s\kappa^2_{j,s}(\gamma_1)+\sum_{j=\floor{ \gamma_2}}^s\kappa^2_{j,s}( \gamma_2)-2\sum_{j=\floor{ \gamma_2}}^s\kappa_{j,s}(\gamma_1)\kappa_{j,s}( \gamma_2)
 \]
Now, for any $\floor{\gamma_1}\leq j \leq s$, define the first derivative
\[
 \dot{\bar\kappa}_{j,s}(\gamma_1)\coloneqq \frac{\sf d}{{\sf d}\gamma_1}\bar\kappa_{j,s}(\gamma_1) = \bar\kappa_{j,s}(\gamma_1) [\psi(j+1-\gamma_1)-\psi(s+1-\gamma_1)+1/\gamma].
\]
\textbf{Claim.} {\it For any $\gamma_1, \gamma_2 \in \Gamma$}
\[
 |\kappa_s(\gamma_1)-\tilde\kappa_s( \gamma_2)|^2 \geq \sum_{j=\floor{ \gamma_2}}^s(\dot{\bar\kappa}_{j,s}( \gamma_2))^2(\gamma- \gamma_2)^2.
\]
{\it and, therefore,}
\[
\ssup\limits_{\theta \in B_{0,\delta}}-{\sf D}_m(\theta) \leq -\delta^2
\]
{\it for $B_{0,\delta} \coloneqq \{\theta \in \Theta: |\theta-\theta_0| < \delta\}$}.
